LiFT: Leveraging Human Feedback for Text-to-Video Model Alignment

Recent advances in text-to-video (T2V) generative models have shown impressive capabilities. However, these models are still inadequate in aligning synthesized videos with human preferences (e.g., accurately reflecting text descriptions), which is particularly difficult to address, as human preferences are subjective and challenging to formalize as objective functions. Existing studies train video quality assessment models that rely on human-annotated ratings for video evaluation but overlook the reasoning behind evaluations, limiting their ability to capture nuanced human criteria. Moreover, aligning T2V model using video-based human feedback remains unexplored. Therefore, this paper proposes LiFT, the first method designed to leverage human feedback for T2V model alignment. Specifically, we first construct a Human Rating Annotation dataset, LiFT-HRA, consisting of approximately 10k human annotations, each including a score and its corresponding rationale. Based on this, we train a reward model LiFT-Critic to learn reward function effectively, which serves as a proxy for human judgment, measuring the alignment between given videos and human expectations. Lastly, we leverage the learned reward function to align the T2V model by maximizing the reward-weighted likelihood. As a case study, we apply our pipeline to CogVideoX-2B, showing that the fine-tuned model outperforms the CogVideoX-5B across all 16 metrics, highlighting the potential of human feedback in improving the alignment and quality of synthesized videos.

==> figs/vidcritic1.tex <==
\begin{figure}[hbt]

    \centering
    \includegraphics[width=1.0\linewidth]{figs/vidcritic.pdf}
    \caption{The training process illustration of VidCritic.}
    \label{fig:appearance_transfer}

\end{figure}


==> tables/dataset_distribution.tex <==
\begin{table}[t]
% \setlength\tabcolsep{2.5pt}
\centering
% \small
\caption{Details of our proposed HFVQA.}

\begin{tabular}{c|cc|cccc}

		\bottomrule
       \multirow{2}{*}{Category}   &  \multicolumn{2}{c|}{Total \# of}& \multicolumn{3}{c}{Human feedback (\%)}
     
       \\
          & types & videos &
	Good
      & Normal
  &Bad

       \\

       		\bottomrule

		
 		Human &23 & 7753    &  35.9       & 14.7     & 49.4    \\

		 Animal& 158 & 8273 &   34.6            & 17.6 &47.8            \\


		
 		Place &179  & 1231    &  37.6       & 17.1     & 45.2     \\

		Easy Act. & 18 & 2046 &   31.4            & 17.8 &50.7           \\
        Complex Act. & 83 & 3968 &   34.9            & 16.9 &48.2           \\
		\bottomrule

	\end{tabular} \\


\label{tab:detail_dataset}
\end{table}


==> tables/design_compare.tex <==
\begin{table*}[t]
\setlength\tabcolsep{4pt}
\centering
\small
\caption{}

\begin{tabular}{ccccccccccc}

		\bottomrule
         Models & \makecell[c]{RM \\ Size} &
	\makecell[c]{Subject\\ Consistency}
      & \makecell[c]{Background\\ Consistency}
  &\makecell[c]{Aesthetic \\Quality} &\makecell[c]{Imaging \\Quality}
&\makecell[c]{Object \\Class}
&\makecell[c]{Multiple \\Objects}
&\makecell[c]{Appearance \\Style}
& \makecell[c]{Human \\Action}

       \\
		\bottomrule

		
 		CogVideoX-2B  &     &  94.58       & 95.45     & 61.94  &63.04 & 85.75 &69.11 &24.67 &97.34    \\

		CogVideoX-5B   &  &   94.84            & 95.64 &\underline{63.13}    &63.14 &88.99 & 70.98 & \underline{24.70}& \underline{98.40}        \\

        \bottomrule
             CogVideoX-2B-SFT      & \multirow{2}{*}{13B}          & 96.01             & 96.39   &62.42   &63.13 &91.08& 74.05 & 24.81& 97.33   \\
          CogVideoX-2B-RW &         & 96.15             & 96.48    &63.24   &64.01 &91.27& 77.45& 24.86 & 97.40   \\

        \bottomrule
             CogVideoX-2B-SFT      & \multirow{2}{*}{40B}          & \underline{96.16}             & \underline{96.58}    &62.82   &\underline{63.37} &\underline{91.39}& \underline{74.50} & 24.34 & 97.00   \\
          \textbf{CogVideoX-2B-RW} &         & \textbf{96.82}             & \textbf{96.79}    &\textbf{63.72}   &\textbf{64.19} &\textbf{91.77}& \textbf{79.34} & \textbf{25.92} & \textbf{98.44}   \\
		\bottomrule

                
		Models  & \makecell[c]{RM \\ Size} &
		\makecell[c]{Color}
       & \makecell[c]{Spatial \\Relationship}
  &\makecell[c]{Scene} &\makecell[c]{Temporal \\Style}
&\makecell[c]{Overall \\Consistency}
&\makecell[c]{Temporal \\Flickering}
&\makecell[c]{Motion \\Smoothness}
& \makecell[c]{Dynamic \\Degree}

       \\
		\bottomrule

		
		CogVideoX-2B &     &  80.86     & 61.78     & 53.30  &24.19 & 27.34 &96.94 &\underline{97.86} &60.22      \\

		CogVideoX-5B   &    &   82.50            & 55.94 &56.57    &\underline{25.12} &\underline{27.84} & 97.19 & 97.81 & 62.78    \\
        \bottomrule
                 CogVideoX-2B-SFT          & \multirow{2}{*}{13B}   &  83.15             & 62.06    &56.12  & 24.34& 27.02& 97.91 & 97.50& 57.22  \\
            CogVideoX-2B-RW    &      & 84.40             & 64.66    &55.76   &24.83 &27.03& 98.10 & 98.17 & 61.89  \\
        \bottomrule
                 CogVideoX-2B-SFT          & \multirow{2}{*}{40B}   &  \textbf{86.12}             & \underline{62.33}    &\underline{57.30}   &24.98 &27.05& \underline{98.04} & 97.85 & \underline{61.11}   \\
            \textbf{CogVideoX-2B-RW}    &      & \underline{85.15}             & \textbf{66.04}    &\textbf{57.63}   &\textbf{25.23} &\textbf{27.93}& \textbf{98.20} & \textbf{98.33} & \textbf{62.85}   \\
		\bottomrule
	\end{tabular} \\


\label{tab:vbench_compare}
\end{table*}


==> tables/genAI_compare.tex <==
\begin{table}[t]
\setlength
\tabcolsep{21pt}
\centering
\small
\caption{\textbf{Preference accuracy on GenAI-Bench}. \textbf{w/ Ties} indicates that accuracy is calculated with ties, and \textbf{w/o Ties} excludes tied pairs when calculating accuracy.}

\begin{tabular}{cccc}

		\toprule
     \multirow{2}{*}{Method} &    \multicolumn{2}{c}{\textbf{GenAI-Bench}} \\
          & w/ Ties & 
	w/o Ties
      

       \\

       		\midrule
          
    Random  &   34.88  &      47.35     \\
   
    VideoScore  & \textbf{52.71}    &    69.09    \\

		\midrule
		
 		\multirow{1}{*}{LiFT-Critic}   & 51.68 &  \textbf{71.82}      \\
		\bottomrule

	\end{tabular} \\
\label{tab:genAI}
\end{table}

